Calibrating Multi-modal Representations: A Pursuit of Group Robustness without Annotations

Fine-tuning pre-trained vision-language models, like CLIP, has yielded success on diverse downstream tasks. However, several pain points persist for this paradigm: (i) directly tuning entire pre-trained models becomes both time-intensive and computationally costly. Additionally, these tuned models tend to become highly specialized, limiting their practicality for real-world deployment; (ii) recent studies indicate that pre-trained vision-language classifiers may overly depend on spurious features -- patterns that correlate with the target in training data, but are not related to the true labeling function; and (iii) existing studies on mitigating the reliance on spurious features, largely based on the assumption that we can identify such features, does not provide definitive assurance for real-world applications. As a piloting study, this work focuses on exploring mitigating the reliance on spurious features for CLIP without using any group annotation. To this end, we systematically study the existence of spurious correlation on CLIP and CLIP+ERM. We first, following recent work on Deep Feature Reweighting (DFR), verify that last-layer retraining can greatly improve group robustness on pretrained CLIP. In view of them, we advocate a lightweight representation calibration method for fine-tuning CLIP, by first generating a calibration set using the pretrained CLIP, and then calibrating representations of samples within this set through contrastive learning, all without the need for group labels. Extensive experiments and in-depth visualizations on several benchmarks validate the effectiveness of our proposals, largely reducing reliance and significantly boosting the model generalization.

==> tables/table1.tex <==
\begin{table}
  \centering
    \caption{Results of fine-tuning CLIP-RN50 with a subset of ImageNet classes, ``baby pacifier" and ``water bottle". Both average and worst-group performance are evaluated with models early stopped at the \textit{highest worst-group accuracy} on the validation set.}
  \begin{tabular}{@{}lcccc@{}}
    \toprule
     Class 680   & \multicolumn{2}{c}{Accuracy} & \multicolumn{2}{c}{AIoU}  \\
     Baby Pacifier & Avg. & Worst & Avg. & Worst \\
    \midrule
    Pre-trained & 73.7\% & 30.8\% & 0.651 & 0.380 \\
    Fine-tuned  &  94.1\% & 91.7\% & 0.650 & 0.571 \\
    \midrule
    ERM & \textbf{94.9\%} & \textbf{96.2\%} & 0.661 & 0.454  \\
    Group DRO & 89.6\% & 93.1\% & 0.661 & 0.568 \\
    Ours($\mathcal{L}_{lc}$+$\mathcal{L}_{vc}$+$\mathcal{L}_{ls}$) & \textbf{94.9\%} & \textbf{96.2\%} & \textbf{0.720} & \textbf{0.645}  \\
    \bottomrule
  \end{tabular}
  \label{tab:all model dataset}
\end{table}

==> tables/table3.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%TABLE_Components%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{table}[ht]
\centering
\caption{Ablation on {\bf (a)} model component: w/o Random Sampled Images (RSI); w/o Local Contrastive Distillation (Stage-$ii$); w/o Anatomical Contrast Fine-tuning (Stage-$iii$); {\bf (b)} loss formulation: w/o $\mathcal{L}_\mathrm{anco}$; w/o $\mathcal{L}_\mathrm{unsup}$;, compared to the Vanilla and our proposed ACTION. Note that $\mathcal{L}_\mathrm{unsup}$ denotes cross-entropy loss (on pseudo-labels generated by a confidence threshold $\theta_s$) together with $\mathcal{L}_\mathrm{anco}$ used in Stage-$iii$.} 
% \vspace{-10pt}
\label{tab:component_ablation}
\resizebox{0.45\textwidth}{!}{
\begin{tabular}{c|l|c c} 
\toprule
& \,\multirow{2}{*}{Method} & \multicolumn{2}{c}{\textbf{Metrics}} \\ 
    & & Dice{[}\%{]}
    & ASD{[}voxel{]} 
    \\ \midrule
    & \,Vanilla  
    & 60.6
    & 6.64
    \\
	& \,ACTION (ours)
    & \textbf{87.5}
    & \textbf{1.12}   
    \\ 
    \midrule
    \multirow{4}{*}{\bf (a)} 
    & \quad w/o RSI
    & 82.7
    & 6.66
    \\
    & \quad w/o Stage-$ii$
    & 86.4
    & 1.69
    \\
    & \quad w/o RSI + Stage-$ii$ \quad
    & 82.6
    & 1.77
    \\
    & 
    \quad w/o Stage-$iii$
    & 76.7
    & 2.91
    \\ \midrule
    \multirow{2}{*}{\bf (b)}
    & \quad w/o $\mathcal{L}_\mathrm{anco}$
    & 86.5
    & 1.30
    \\
    &   
    \quad w/o $\mathcal{L}_\mathrm{unsup}$ 
    & 83.7
    & 2.51
    \\ 
    \bottomrule
\end{tabular}
}
% \vspace{-15pt}
\end{table}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%TABLE_Components%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

